supDQN: Supervised Rewarding Strategy Driven Deep Q-Network for sEMG Signal Decontamination

The presence of muscles throughout the active parts of the body such as the upper and lower limbs, makes electromyography-based human-machine interaction prevalent. However, muscle signals are stochastic and noisy. These noises can be regular and irregular. Irregular noises due to movements or electrical switching require dynamic filtering. Conventionally, filters are stacked, which trims and delays the signal unnecessarily. This study introduces a decontamination technique involving a supervised rewarding strategy to drive a deep Q-network-based agent (supDQN). It applies one of three filters to decontaminate a 1sec long surface electromyography signal, which is dynamically contaminated. A machine learning agent identifies whether the signal after filtering is clean or noisy. Accordingly, a reward is generated. The identification accuracy is enhanced by using a local interpretable model-agnostic explanation. The deep Q-network is guided by this reward to select filter optimally while decontaminating a signal. The proposed filtering strategy is tested on four noise levels (-5 dB, -1 dB, +1 dB, +5 dB). supDQN filters the signal desirably when the signal-to-noise ratio (SNR) is between -5 dB to +1 dB. It filters less desirably at high SNR (+5 dB). A normalized root mean square (nRMSE) is formulated to depict the difference of filtered signal from ground truth. This is used to compare supDQN and conventional methods including wavelet denoising with debauchies and symlet wavelet, high order low pass filter, notch filter, and high pass filter. The proposed filtering strategy gives an average value nRMSE of 1.1974, which is lower than the conventional filters.

==> figure_tex/ablation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/ablation.pdf}
    \caption{\textbf{(Left) Orthogonal adaptation.} Enforcing row-space orthogonality between style and content LoRA improves image quality, where the images capture the style better and have fewer visual artifacts. \textbf{(Right) Style guidance.} We compare style control capabilities between our style guidance and standard LoRA weight scaling~\cite{dreamboothlora}. \textbf{{\color{MyDarkBlue} Blue}} and \textbf{{\color{MyDarkGreen} green}} stand for the LoRA weight scale and style guidance scale, respectively. Style guidance better preserves content when the style is applied. More details of style guidance formulation are in Section~\ref{sec:cfgstyle}.}
    \label{fig:ablation}
    \vspace{-10pt}
\end{figure}


==> figure_tex/baselines_style_guid.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/baselines_style_guid.pdf}
    \caption{\maxwellchange{Result of our method compared to the strongest baselines, but replacing LoRA scale (Eq. \ref{eq:oldinference}) with our style guidance (Eq. \ref{eq:newinference}) for the baselines. While our style guidance increases baseline performance over LoRA scale images displayed in Figure \ref{fig:main_result}, our method is still superior in terms of preserving content while applying style.}}
    \label{fig:baseline_style_guid}
        \vspace{-10pt}

\end{figure*}


==> figure_tex/blending.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/blending_v2.pdf}
        \vspace{-5pt}
    \caption{\textbf{Blending multiple style guidances.} We can compose multiple customized models by directly blending each style guidance together. Adjusting blending strength of each model allows us to acquire a smooth style transition. Train Image Pair 0 Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}}
    \label{fig:blending}
    \vspace{-10pt}
\end{figure}


==> figure_tex/limitation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/limitation.pdf}
    \caption{\textbf{Limitations.} \emph{Left}: 
     our method struggles with categories when they significantly differ from the training categories. Here, our method fails to transfer the artistic style of landscape image pairs to human portraits. \emph{Right}: our method can cause structure changes in some instances, like change of body position or background changes.
    }
    \label{fig:limitation}
    \vspace{-10pt}
\end{figure}


==> figure_tex/main_figure.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/main_results_v7.pdf}
    \caption{Result of our method compared to the strongest baselines.
    \maxwellchange{When only training with the style image as in DB LoRA, the image structure is not preserved and overfitting occurs. While Concept Slider's training scheme~\cite{gandikota2023concept} uses both style and content images, it still exhibits overfitting and loss of structure in many cases.} Our method preserves the structure of the input mage while faithfully applying the desired style. We use style guidance strength 3 and classifier guidance strength 5.
    Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse} (Third row) and \href{https://www.instagram.com/aaronhertzmann/?hl=en}{Aaron Hertzmann} (Fourth row)}
    \label{fig:main_result}
\end{figure*}


==> figure_tex/method.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/method_v7.pdf}
        \vspace{-5pt}
    \caption{\textbf{Method overview}. (Left) We disentangle style and content from an image pair by jointly training two low-rank adapters, StyleLoRA and ContentLoRA, representing style and content, respectively. Our training objective consists of two losses: The first loss fine-tunes ContentLoRA to reconstruct content image conditioned on a content prompt. The second loss encourages reconstructing the style image using \textit{both} StyleLoRA and ContentLoRA conditioned on a style prompt, but we only optimize Style LoRA for this loss. (Right) At inference time, we only apply StyleLoRA to customize the model. Given the same noise seed, the customized model generates a stylized counterpart of the original pre-trained model output. {\menlo V*} is a fixed random rare token that is a prompt modifier for the content image. Style image credits: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}}
    \label{fig:method}
        \vspace{-10pt}
\end{figure*}



==> figure_tex/mturk.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=.7\textwidth]{figure_pdf/turk_image.pdf}
    \caption{Mturk User Interface
    }

    \label{fig:mturk}
        \vspace{-10pt}
\end{figure}


==> figure_tex/teaser.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/teaser_jack_dog_v2.pdf}
        \vspace{-5pt}
    \caption{%
    Given a \emph{single} image pair, we present \methodname, a method for customizing a pre-trained text-to-image model and learning a new style from the image pair's stylistic difference. Our method can apply the learned stylistic difference to new input images while preserving the input structure. Compared to Dreambooth LoRA\cite{hu2022lora, loraimplementation}, a standard customization method that solely use style images, our method effectively disentangles style and content, resulting in better structure, color preservation, and style application. Style image credit: \href{https://www.instagram.com/parkhouse_art/}{Jack Parkhouse}.
    }
    \label{fig:teaser}
        \vspace{-15pt}
\end{figure*}



==> figure_tex/tradeoff_plot.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure_pdf/quantitative_analysis_sliders.pdf}
    \caption{\textbf{Quantitative comparison with baselines on learned style.} Given a fixed inference path, our method's pareto dominates baselines for image generation both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right). \maxwellchange{Secondly, our proposed style guidance outperforms standard LoRA weight scale guidance for our training method (blue vs. orange), DB LoRA (green vs. pink), and Sliders (brown vs. purple)}. In the Appendix's Figure \ref{fig:tradeoff_plot_diversity}, we further evaluate the diversity of generated images. We show that baselines often lose diversity, while our method leads to diverse generations while still achieving lower perceptual distance to the ground truth style.
    Increased marker size corresponds to an increase in style guidance scale.
    }
    \label{fig:tradeoff_plot}
\end{figure*} 






==> figure_tex/tradeoff_plot_diversity.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/sliders_diversity.pdf}
    \caption{\textbf{Quantitative comparison on Diversity metric.} Our method with style guidance has high diversity and low perceptual distance to ground truth style images both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right). 
    Methods without edge control tend to lose diversity indicating overfitting, and methods with edge control have similar/higher diversity, but much worse style application.  
    Increased marker size corresponds to an increase in style guidance scale.
    }
    \label{fig:tradeoff_plot_diversity}
\end{figure*} 






==> figure_tex/tradeoff_plot_diversity_style_aligned.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/tradeoff_plot_diversity_style_aligned.pdf}
    \caption{\textbf{Image diversity with Style Aligned \cite{hertz2023style} on learned style (Diversity).} Our method has high diversity and low perceptual distance to ground truth style images both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right) as compared to both versions of Style Aligned Image Generation. 
    }
    \label{fig:tradeoff_plot_diversity_style_aligned}
\end{figure*} 






==> figure_tex/tradeoff_plot_style_aligned.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure_pdf/tradeoff_plot_style_aligned.pdf}
    \caption{\textbf{Style similarity with Style Aligned \cite{hertz2023style}.} Our method Pareto dominates both versions of Style Aligned Image Generation for image generation both on the same category as training (left) and when evaluated on categories different from training, e.g., trained on human portraits but tested on dog images (right).
    }
    \label{fig:tradeoff_plot_style_aligned}
\end{figure*} 






==> figure_tex/training_data.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figure_pdf/training_data.pdf}
    \caption{\textbf{Training Data.} We present the synthetic training data set used for evaluation, where each pair is used as a single training instance. Each column corresponds to a different style, and each row corresponds to a different content category.}
    \label{fig:training_data}
\end{figure*}

